Rethinking Social Robot Navigation: Leveraging the Best of Two Worlds

Empowering robots to navigate in a socially compliant manner is essential for the acceptance of robots moving in human-inhabited environments. Previously, roboticists have developed geometric navigation systems with decades of empirical validation to achieve safety and efficiency. However, the many complex factors of social compliance make geometric navigation systems hard to adapt to social situations, where no amount of tuning enables them to be both safe (people are too unpredictable) and efficient (the frozen robot problem). With recent advances in deep learning approaches, the common reaction has been to entirely discard these classical navigation systems and start from scratch, building a completely new learning-based social navigation planner. In this work, we find that this reaction is unnecessarily extreme: using a large-scale real-world social navigation dataset, SCAND, we find that geometric systems can produce trajectory plans that align with the human demonstrations in a large number of social situations. We, therefore, ask if we can rethink the social robot navigation problem by leveraging the advantages of both geometric and learning-based methods. We validate this hybrid paradigm through a proof-of-concept experiment, in which we develop a hybrid planner that switches between geometric and learning-based planning. Our experiments on both SCAND and two physical robots show that the hybrid planner can achieve better social compliance compared to using either the geometric or learning-based approach alone.

==> content/backup.tex <==
The essential goal of navigation parameter selection is to find a mapping $f : \mathcal{X} \rightarrow \Theta$, where $\mathcal{X}$ denote the space of possible inputs of any navigation system, and $\Theta$ is the parameter space. Since most navigation systems like ROS involves highly complex procedures to plan and perform actions, we do not want to put too much assumptions on $f$. In this work, we only assume that parameters are clustered in modes, which matches with real-life observations, and $f$ can be evaluated via sampling. By doing so, we treat $f$ as a compositional function:
\begin{equation}
    f(x) = h \circ g(x),
\end{equation}
where $g_\phi: \mathcal{X} \rightarrow \mathcal{Z}$ is a parameterized function that maps the local context to a specific parameter category and $h: \mathcal{Z} \rightarrow \Theta$ acts like a dictionary that selects the right parameter given a category from $\mathcal{Z}$. By dividing $f$ into these two functions, learning can be done separately for each of them. In particular, to learn $g$, we collect supervised data along sampled trajectories where the labels of regions are provided by a human expert watching those trajectories. To build the dictionary $h$, we use CMA-ES, a sampling based black-box optimization technique to find a near optimal set of parameters that best imitates the expert trajectory. To measure the closeness between the expert trajectory and the simulated trajectory from the robot, we first define a set of way points and then use the sum of mean square errors between these way points as the final cost that CMA-ES minimizes.

To further stabilzie the mode selection and incorporte the history into consideration, we enrich the formulation of $g$ by adopting a simple but powerful model called Hidden Markov Model (HMM). Essentially, we are performing Bayesian filtering at each time $t$ based on the past observations. The resulting formula of $g(x_t)$ then becomes:

\begin{equation}
    g(x_t | y_1, \dots, y_t) = p(x_1) \underbrace{ \prod_{k=1}^{t-1} p_{\phi_e}(x_{k+1} | x_k)}_{\text{transition probability}} \overbrace{\prod_{k=1}^t p_{\phi_o}(y_k | x_k)}^{\text{emission probability}}
\end{equation}

During practice, we can train parameterized models $p_{\phi_e}$ and $p_{\phi_o}$ by maximizing the likelihood of the observations (via the forward algorithm) on the labeled data.
\vspace{-10pt}
\begin{figure}[h!]
  \centering
  \tikz{ %
    \node[latent] (x1) {$x_1$} ; %
    \node[latent, right=of x1] (x2) {$x_2$} ; %
    \node[latent, right=of x2] (x3) {$x_3$} ; %
    \node[latent, right=of x3] (xt) {$x_t$} ; %

    \node[latent, below=of x1] (y1) {$y_1$} ; %
    \node[latent, right=of y1] (y2) {$y_2$} ; %
    \node[latent, right=of y2] (y3) {$y_3$} ; %
    \node[latent, right=of y3] (yt) {$y_t$} ; %

    \edge {x1} {y1} ; %
    \edge {x2} {y2} ; %
    \edge {x3} {y3} ; %
    \edge {xt} {yt} ; %
    \edge {x1} {x2} ; %
    \edge {x2} {x3} ; %
    % \edge {x} {s2} ; %
    % \edge {s2} {s3} ; %

    % \path (s1) edge [bend right=50,->]  (o1) ; %
    % \path (s2) edge [bend right=50,->]  (o2) ; %
    % \path (s3) edge [bend right=50,->]  (o3) ; %
    % \path (st) edge [bend right=50,->]  (ot) ; %
    \path (x3) -- node[auto=false]{\ldots} (xt);
  }
  \caption{A graphical model representation of the Hidden Markov Model. In our case, $x_t$ represent the latent mode of different scenarios at time $t$, while $y_t$ denote the sensory input at time $t$.}
  \label{fig:graphical_model}
  \vspace{20pt}
\end{figure}


% where $\tilde{s_i}$ denotes the $i$th state on the demonstrator's trajectory and $\tilde{a_i}$ the $i$th action from the demonstrator. The policy $\pi_{\theta}(\cdot | \cdot)$ is any navigation stack parameterized by $\theta$ and gives the probability of taking a particular action based on the current state. Due to different characteristics of various navigation algorithms, the state $s_i$ is loosely defined as all necessary information for the planner to determine its action $a_i$ at time $i$. This is particularly important because many planners are not strictly memory-less, and their necessary memory to determine current action is factored into this state, e.g. history costmap, previous position, velocity, acceleration, etc. Action $a_i$ depends on the type of the robot, and for most nonholonomic ground robots, $a_i = (v, \omega)$, where $v$ and $\omega$ are linear and angular velocities, respectively. 

% The proposed framework does not rely on any assumptions of the underlying navigation algorithm $\pi_{\theta}(\cdot | \cdot)$, but being able to sample from the planner. Given a state $\tilde{s_i}$ on the demonstrator's trajectory (which may contain history necessary for the planner to induce an action), action $a_i$ is sampled from querying the navigation algorithm. Mean Squared Error (MSE) is used to quantify the difference between sampled $a_i$ and demonstrator action $\tilde{a_i}$. To cope with different control frequencies from demonstration and navigation, a loss metric shown in Fig.~\ref{fig:mse} is used, which is a special case of Dynamic Time Warping approach \cite{berndt1994using}: for every demonstrator action, the closest navigation action before it is found and MSE is calculated based on this pair of actions. If the duration between this pair of actions is greater than a constant \emph{execution time}, i.e. no new navigation action is computed in time causing the robot to stall, error with respect to zero will be calculated. 


% APPROACH
% In this section, the proposed framework is presented in a bottom-up order: Firstly, Behavior Cloning to match navigation with human demonstration given a specific region is introduced, autonomously finding parameters specifically tailored for the characteristics of this region. As to be shown in Sec.~\ref{sec::experiments}, while working well in the dedicated region, overall performance suffers from applying the same set of parameters all over the entire environment. Therefore, an unsupervised environment context classifier based on change point detection is secondly introduced, dividing the entire environment into different context regions, for whom specific parameters could be learned from Behavior Cloning. The unsupervised change point detection technique does not assume the human demonstrator has knowledge about different navigational contexts. 

% This section first formalizes the problem definition and introduces all relevant notations, and then presents the proposed framework in a bottom-up order: firstly, assume the underlying environment consists of one single context, Behavior Cloning with black-box optimization is applied to find a single set of planner parameters that best imitates the human demonstration; Then, the above method is treated as a sub-procedure for a more general framework that can automatically detect different contexts within a single demonstration and learn the corresponding parameters. In addition, a context predictor is introduced for autonomously switching planner parameters online during the run time.

% Given a navigation stack $G$ and a new environment $\mathcal{E}$, a set of pre-tuned (default) parameters may generate sub-optimal behaviors, e.g., frequently getting stuck, moving too slow/fast, over-/under-react to the presence of obstacles, etc. However, human demonstrator can easily tele-operate the robot to navigate through unseen environment in a desirable manner. Therefore, Behavior Cloning (BC) is adopted to find the optimal parameters to approximate human demonstration. Formally, denote the single-shot demonstration as a time series $\{t^D_i, a^D_i, x^D_i\}_{i=1}^N$, where $t^D_i$ is time, $a^D_i = (v^D_i, \omega^D_i)$ is demonstration output, i.e. the velocity and angular velocity, and $x^D_i$ is an abstract state that encodes everything on which the navigation stack is conditioned to output an action, assuming the navigation is running in the background during demonstration but does not output actions. Here $(\cdot)^D$ emphasizes $(\cdot)$ is from demonstration. In particular, denote $l^D_i \in x^D_i$ as the LiDAR inputs at time step $i$. Furthermore, assume the navigation stack $G$ has a set of tunable parameters $\theta \in \Theta$, then the behavior cloning objective is to find an optimal $\theta$ that maximizes the likelihood of the demonstration: 
















% We now describe our approach for tuning a black-box robotic navigation system using a human-teleoperated demonstration.
% We will introduce our approach into two stages.
% In the first stage, we formulate the navigation system tuning from demonstration problem for relatively uniform environments in which we expect an unknown but fixed set of system parameters will suffice, and we then present a procedure by which a demonstration may be used to automatically infer those parameters.
% In the second stage, we extend our formulation to more dynamic environments in which we expect that different system parameters will be required in different contexts (i.e,. regions of the environment), and we present a procedure by which these contexts can be inferred and demonstration data can be used to automatically find the system parameters for each context.
% Overall, we refer to our approach as {\em navigation system tuning from demonstration} (NSTfD) \bo{we need to finalize the acronym}.
% A block diagram of the approach is given in Fig. \garrett{insert figure ref here---you can ref a block diagram on page 1 like peter suggested}, and the overall algorithm is specified in Algorithm~\ref{alg:apparent}.
% \garrett{given that i made the old "problem definition" section much longer, i removed the setup paragraph here so we could dive right in. please review and let me know what you think}

% When a robot is navigating in a new environment $\mathcal{E}$, a set of pre-tuned (default) parameters may generate sub-optimal behaviors, e.g., frequently getting stuck, moving too slow/fast, over-/under-react to the presence of obstacles, etc. However, human demonstrator can easily tele-operate the robot to navigate through unseen environment in a desirable manner. Therefore, APPLD is developed to enable efficient parameter adaptation in a new environment with a single human demonstration.

% In this section, we formalize the problem definition of APPLD and present the proposed learning framework in a bottom-up order. Specifically, behavior cloning a single set of parameter is introduced for planner parameter optimization in environments with relatively similar scenarios, which we call the context. Then, the above method is treated as a sub-procedure for a more general framework that can automatically detect different contexts within a single demonstration and learn the corresponding parameters.

% As input to CHAMP, we provide the LiDAR range data and the demonstrated actions $\{l^D_i, a^D_i\}_{i=1}^N$.
% \garrett{the above needs to instead be formulated with respect to $x$, and then you can explain how lidar is a part of $x$.}
% For faster computation, LiDAR sensory inputs are treated as a distribution and low order moments (mean $\mu_{\text{LiDAR}}$ and standard deviation $\sigma_{\text{LiDAR}}$) are taken as the relevant statistics to summarize the whole LiDAR input.
% CHAMP requires a model, $Q$, to be associated with each segment that functions as a probabilistic generative model for the inputs.
% For simplicity, we used in our work a four-dimensional Gaussian distribution ($\mu_{\text{LiDAR}}$, $\sigma_{\text{LiDAR}}$, $v$, $\omega$).
% \garrett{as with the comment about lidar, the above needs to be formulated with $a$ and then you can explain how $v$ and $\omega$ are the components in our work.}
% With this specific configuration, given the input sequence $\{l^D_i, a^D_i\}_{i=1}^N$, CHAMP outputs a sequence of changepoints $\tau_1, \tau_2, \dots, \tau_{K-1}$ so that the demonstration is chunked into $K$ segments, each with uniform context.



% BELOW ARE THE OLD APPROACH

\section{Adaptive Planner Parameters Learning from Demonstration}
\label{sec::approach}
In the following, we formalize the problem definition and present the developed method in a bottom-up order.

\subsection{Problem Definition}
We assume that we are given a robot with its navigation planner $G: \mathcal{X} \times \Theta \rightarrow \mathcal{A}$, where $\mathcal{X}$ represents the state space of the planner (e.g., current position of the robot, the position of nearby obstacles, information about the current local navigation goal, etc.), $\Theta$ represents the space of free parameters for $G$ (e.g., sampling density, maximum velocity, etc.), and $\mathcal{A}$ represents the planner's action space (e.g., commanded linear and angular velocity).
Using $G$ and a particular parameter set $\theta$, the robot performs navigation by repeatedly estimating its state $x$ and applying action $a = G(x;\theta) = G_\theta(x)$.
Importantly, we do not assume that we have any access to or knowledge of the inner workings of $G$ other than that we can specify local navigation goals (which we encode in $x$), and that we can induce some sort of behavior change by modifying $\theta$.
In other words, $G$ is a black-box planner, e.g., we do not assume that it is differentiable, and we need not even understand what each component of $\theta$ does.

Given $G$, the problem we consider in this paper is that of \emph{determining a parameter-selection strategy that will lead to successful navigation}, i.e., parameters that allow the robot to move towards its goal quickly and smoothly.
We approach this problem as one of learning from human demonstration, i.e., we assume that a human can provide a tele-operated demonstration of successful navigation behavior in the deployment environment, and we then seek a selection scheme for $\theta$ that can produce navigation behavior like the demonstration.
More formally, we assume that, during human teleoperation, we can record a demonstration $\mathcal{D} = \{ x^D_i, a^D_i, t^D_i \}_{i=1}^N$, where $N$ is the total number of recorded state-action pairs, and $x^D_i$ and $a^D_i$ represent the robot state and demonstrated action at time $t^D_i$.
Given $\mathcal{D}$, the particular problem we consider in this paper is that of finding two functions: \textbf{(1)} a mapping $M: \mathcal{C} \rightarrow \Theta$ that determines planner parameters for a given {\em context} $c$, and \textbf{(2)} a parameterized context predictor $B_\phi: \mathcal{X} \rightarrow \mathcal{C}$ that predicts the context given the current state.
Given $M$ and $B_\phi$, our system performs navigation by selecting actions according to $G(x; M(B_\phi(x)))$.
Importantly, the formulation presented here involves only changing the {\em parameters} of $G$, i.e., the learned navigation strategy will still possess the benefits that many modern $G$ can provide such as safety guarantees.

\subsection{Learning for a Single Context}
\label{subsec:single}
In the case of a single context (i.e., when the robot's environment is relatively uniform), we assume that a single set of parameters suffices for robust navigation.
The learning problem then reduces to that of finding a constant mapping $M=\theta^* \; \forall x$.
To find this $\theta^*$, we employ {\em behavioral cloning} (BC) \cite{pomerleau1989alvinn}, i.e., we seek to minimize the difference between the demonstrated actions and the actions that $G_{\theta^*}$ would produce.
More specifically,

\begin{equation}
    \begin{split}
    \theta^* &= \argmin_{\theta} \sum_{i=1}^N ||a^D_i - G(x^D_i; \theta))||_H,
    \end{split}
    \label{eqn:bc}
\end{equation}
where $||\cdot||_H$ is the induced norm by a diagonal matrix $H$ with positive real entries, which is used for weighting each dimension of the action. A black-box optimization method $A_{\text{black-box}}$ is then applied to solve Equation~\ref{eqn:bc}.

\subsection{Identifying and Learning across Multiple Contexts}
As we will show in Section~\ref{sec::experiments}, when faced with a complex environment, the human demonstrator needs to drive the robot differently in different regions of the state space such that no single set of planner parameters $\theta$ can closely approximate the demonstration in all states.
In order to overcome this problem, our technique employs dynamic, context-dependent parameter switching, which consists of three stages: \textbf{(a) }{\em demonstration segmentation}, in which we seek to identify context switching within the demonstration, \textbf{(b) }{\em parameter learning}, in which we seek to find an optimal set of parameters for individual segment, and \textbf{(c) }{\em online context prediction}, in which we seek to recognize the context and apply the corresponding learned parameters during execution.

\textbf{Demonstration Segmentation:}
% We posit that the human demonstrator qualitatively shifts their navigation behavior based on the current context but, within a given context, the strategy described in Section~\ref{subsec:single} will allow the planner to generate human-like behavior.
The idea of segmentation is to truncate the demonstration into pieces that correspond to a single context only, so that the strategy described in Section~\ref{subsec:single} can then be applied for individual segment.
This is exactly the problem of changepoint detection \cite{adams2007bayesian}.
Given $\mathcal{D} = \{ x^D_i, a^D_i, t^D_i \}_{i=1}^N$, a changepoint detection algorithm $A_{\text{segment}}$ is applied to automatically detect how many changepoints exist and where those changepoints are in the demonstration.
Denote the number of changepoints found by $A_{\text{segment}}$ as $K-1$ and the changepoints as $\tau_1, \tau_2, \dots, \tau_{K-1}$ with $\tau_0 = 0$ and $\tau_K = N$, the demonstration $\mathcal{D}$ is then truncated into $K$ pieces $\{\{x^D_i, a^D_i, t^D_i \,|\, \tau_{k-1} \leq i < \tau_k\}\}_{k=1}^K$.

\textbf{Parameter Learning:} Following demonstration segmentation, we apply the method in Section~\ref{subsec:single} to learn a suitable set of parameters $\theta^*_k$ for each segment $\{x^D_i, a^D_i, t^D_i \,|\, \tau_{k-1} \leq i < \tau_k\}$. Therefore, we form the mapping $M$ as $M(k) = \theta^*_k$.

\textbf{Online Context Prediction:}
In order to select the appropriate parameters during execution, we must be able to predict which context the robot is in from its estimated state $x$.
To do so, we first learn a parameterized function $f_\phi(x)$ using supervised learning, where $f$ seeks to classify which segment of the training data $x^D_i$ came from, i.e., 
\begin{equation}
    \phi^* = \argmax_\phi \sum_{i=1}^N c_i^T \log f_\phi(x^D_i),
\end{equation}
where $c_i$ is the one-hot vector that denotes the ground truth context of $x^D_i$, i.e. $c_i = \bm{e_k}$ if $\tau_{k-1} \leq i \leq \tau_k$.
Given $f_\phi$, we define our context predictor $B$ according to
\begin{equation}
    B_\phi(x_t) = \argmax_c \sum_{i = t-p+1}^t \mathbbm{1}\big[(\argmax_{c'} f_\phi(x_i)) = c\big] \; ,
    \label{eqn:mode_switching}
\end{equation}
In other words, $B_\phi$ acts as a low-pass filter on the context predictions generated by $f_\phi$ over a sliding window of length $p$.

\commentp{Did we say somewhere that CHAMP can determine K on its own?  K appears in Algorithm 1 without any definition of it.  Is it assumed to be an output of $A_{segment}$?  If so, we should make sure that's clear.}

Taken together, the above steps constitute our proposed approach: {\em adaptive planner parameter learning from demonstration} (APPLD). During training, the above three stages are applied sequentially to learn a set of $\{\theta^*_k\}_{k=1}^K$ and a context predictor $B_\phi$. During execution, Equation~\ref{eqn:mode_switching} is applied online to pick the right set of parameters for navigation. Algorithm~\ref{alg:apparent} summarizes the entire pipeline from offline training to online execution.

\begin{algorithm}[ht]
\small
\caption{Adaptive Planner Parameter Learning from Demonstration} \label{alg:apparent}
\begin{algorithmic}[1]
    \STATE{// Training}
    \STATE{\textbf{Input:} the demonstration $\mathcal{D} = \{ x^D_i, a^D_i, t^D_i \}_{i=1}^N$, space of possible parameters $\Theta$, and the navigation stack $G$}.
    \STATE Call $A_{\text{segment}}$ to detect changepoints $\tau_1, \dots, \tau_{K-1}$ with $\tau_0=0$ and $\tau_K=N$.
    \STATE Partition $D$ into $K$ segments $\{\{x^D_i, a^D_i, t^D_i \,|\, \tau_{k-1} < i \leq \tau_k\}\}_{k=1}^K$ with corresponding contexts $\{ c_k \}_{k=1}^K$
    \STATE Use $\{x^D_i, c_i\}_{i=1}^N$ to train $f_\phi$ for context prediction.
    \FOR{$k=1:K$}
        \STATE Call $A_{\text{black-box}}$ with objective defined in Equation~\ref{eqn:bc} on data $\{ x^D_i, a^D_i, t^D_i | \tau_{k-1} \leq i < \tau_k\}$ to find parameters $\theta^*_k$.
    \ENDFOR
    \STATE 
    \STATE{// Deployment}
    \STATE \textbf{Input:} a library of $\{\theta^*_k\}_{k=1}^K$, the navigation stack $G$, and the context predictor $B_\phi$.
    \FOR{$t=1:T$}
        \STATE Change the parameters of $G$ according to Equation~\ref{eqn:mode_switching}.
    \ENDFOR
\end{algorithmic}
\end{algorithm}

